Self-Supervised Learning to Prove Equivalence Between Straight-Line Programs via Rewrite Rules

We target the problem of automatically synthesizing proofs of semantic equivalence between two programs made of sequences of statements. We represent programs using abstract syntax trees (AST), where a given set of semantics-preserving rewrite rules can be applied on a specific AST pattern to generate a transformed and semantically equivalent program. In our system, two programs are equivalent if there exists a sequence of application of these rewrite rules that leads to rewriting one program into the other. We propose a neural network architecture based on a transformer model to generate proofs of equivalence between program pairs. The system outputs a sequence of rewrites, and the validity of the sequence is simply checked by verifying it can be applied. If no valid sequence is produced by the neural network, the system reports the programs as non-equivalent, ensuring by design no programs may be incorrectly reported as equivalent. Our system is fully implemented for one single grammar which can represent straight-line programs with function calls and multiple types. To efficiently train the system to generate such sequences, we develop an original incremental training technique, named self-supervised sample selection. We extensively study the effectiveness of this novel training approach on proofs of increasing complexity and length. Our system, S4Eq, achieves 97% proof success on a curated dataset of 10,000 pairs of equivalent programs.

==> old-text.tex <==
We create one final test dataset $X$ which checks programs found on GitHub with other GitHub programs for a match. In order to train with the GitHub distribution, we need known equivalent pairs which we can search for equivalence hence we create a dataset $C$ of equivalent samples from the GitHub code using compiler steps. The rewrite rules must be discovered by a partially trained model and the rules found can be used to further improve the model, as discussed in section~\ref{sec:incrementallearning}.

To create an initially successful model which can be used to find rewrite rule sequences in $C$, we need pairs of equivalent programs and the rewrite rule sequence which transforms the first program into the semantically equivalent target program. We generate this data in a synthetic manner. 

We call the datasets we use for training $T_n$ where $n$ specifies the stage of incremental learning the set is used for. In particular, $T_0$ is made up solely of samples derived from $R$, while $T_1$ includes samples derived from proofs found between pairs from $R$ and $C$.



